Vision-Based Cooperative MAV-Capturing-MAV

MAV-capturing-MAV (MCM) is one of the few effective methods for physically countering misused or malicious MAVs.This paper presents a vision-based cooperative MCM system, where multiple pursuer MAVs equipped with onboard vision systems detect, localize, and pursue a target MAV. To enhance robustness, a distributed state estimation and control framework enables the pursuer MAVs to autonomously coordinate their actions. Pursuer trajectories are optimized using Model Predictive Control (MPC) and executed via a low-level SO(3) controller, ensuring smooth and stable pursuit. Once the capture conditions are satisfied, the pursuer MAVs automatically deploy a flying net to intercept the target. These capture conditions are determined based on the predicted motion of the net. To enable real-time decision-making, we propose a lightweight computational method to approximate the net motion, avoiding the prohibitive cost of solving the full net dynamics. The effectiveness of the proposed system is validated through simulations and real-world experiments. In real-world tests, our approach successfully captures a moving target traveling at 4 meters per second with an acceleration of 1 meter per square second, achieving a success rate of 64.7 percent.

==> before_document.tex <==

\usepackage{upgreek}
\usepackage{subfig}
\usepackage{amsmath} % use for align
\usepackage{amssymb}
%\usepackage{subfloat}
\usepackage{hyperref}
\usepackage{graphicx,color}
\usepackage{mathrsfs}
\usepackage{cite}
\usepackage{url}
\usepackage{soul}
\usepackage{booktabs}
\usepackage{array}
\usepackage[table]{xcolor}

%\usepackage{bm}
\usepackage{tikz}
\usetikzlibrary{calc} % for calculation functions in Tikz let, in commands in Tikz
\usetikzlibrary{shapes} % for block diagram
\usetikzlibrary{chains}
\usetikzlibrary{fit}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.text} % text along path
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing} % for zigzag arrow
\usetikzlibrary{shadows}
\usetikzlibrary{patterns}
\usetikzlibrary{matrix}
\usepackage{pgfplots}
\usepackage[europeanresistors]{circuitikz}
\usepackage[outline]{contour} % white surround text
\contourlength{1.5pt}
\usepackage{arydshln}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}

\newcommand{\acc}{\mathbf{a}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\bvec}{\mathbf{b}}

\newcommand{\E}{\mathbb{E}}
\newcommand{\e}{\mathbf{e}}

\newcommand{\F}{\mathbf{F}}

\newcommand{\G}{\mathcal{G}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathbf{K}}


\newcommand{\M}{\mathbf{M}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\s}{\mathbf{s}}

\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\vel}{\mathbf{v}}
\newcommand{\W}{\mathbf{W}}

\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}


\renewcommand{\u}{\mathbf{u}}

\newcommand{\bOmega}{\bm{\Omega}}



\newcommand{\Eta}{\boldsymbol{\eta}}

\newcommand{\I}{\mathbf{I}}
\newcommand{\zeros}{\mathbf{0}}

\renewcommand{\H}{\mathbf{H}}
\renewcommand{\L}{\mathcal{B}}
\renewcommand{\P}{\mathbf{P}}
\renewcommand{\S}{\mathbf{S}}
\newcommand{\xe}{x_{\text{e}}}
\newcommand{\sk}[1]{\left[#1\right]_\times} % skew symmetric operator
\newcommand{\dia}[1]{\mathrm{diag}\left(#1\right)} % block diagnal matrix
\newcommand{\Db}{D_{\bar{b}}}
\newcommand{\smin}{\sigma_{\min}}
\graphicspath{{figures/}}

\newcommand{\blue}{\textcolor{blue}}
\renewcommand{\O}{\Omega}
\newcommand{\Obar}{\bar{\Omega}}
\newcommand{\sat}{\mathrm{sat}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\red}{\textcolor{red}}

